Equidistribution for higher-rank Abelian actions on Heisenberg nilmanifolds

We prove quantitative equidistribution results for actions of Abelian subgroups of the $2g+1$ dimensional Heisenberg group acting on compact $2g+1$-dimensional homogeneous nilmanifolds. The results are based on the study of the $C^\infty$-cohomology of the action of such groups, on tame estimates of the associated cohomological equations and on a renormalisation method initially applied by Forni to surface flows and by Forni and the second author to other parabolic flows. As an application we obtain bounds for finite Theta sums defined by real quadratic forms in $g$ variables, generalizing the classical results of Hardy and Littlewood \cite{MR1555099, MR1555214} and the optimal result of Fiedler, Jurkat and K\"orner \cite{MR0563894} to higher dimension.

==> sect6.tex <==
\section{Equidistribution}

We work in $L^2_{\neq 0}(M)$. Therefore, the irreducible components in the
orthogonal decomposition \eqref{orthogonal_decomposition} are all Scr\" odinger
representations $\Sc^\hbar$ with $\hbar \in \Z \backslash \{ 0 \}$ (each one
occurring with multiplicity $|\hbar|$).

\paragraph{Lyapunov coefficients of the renormalization flow on closed
  currents.}

\cyan{(the same argument as ~\cite{MR2218767} Proposition 4.8 gives)} For
$\lambda \in \Lambda(g,d)$, with $1\leq d \leq g$, let $G=G_\lambda \subset
\Hei$ be the isotropic subgroup of coordinate type of dimension $d$, and let
$\alpha \in \Auto$. Let $\beta _\lambda^t$ denotes the renormalization flow
associated to $G_\lambda$, defined in \eqref{renormalization_flow}. The
renormalization flow acts (on the right) on the Sobolev bundle $\bigwedge ^d
\alpha \frak g \otimes \Sobolev^{-s}_\alpha (\Mod)$ of $\alpha \frak
g$-currents of dimension $d$ and Sobolev order $|s|$ according to
\[
\GMod (\alpha , T) \, \mapsto \, \GMod (\alpha \beta_\lambda^t , T)
\]
Recall that the space $\mathcal B_d (\alpha \frak g, M)$ of closed $\alpha
\frak g$-currents is made of $\alpha \frak g$-currents of Sobolev order
$>g/2$. We may therefore consider, for any $s > g/2$, the bundle of closed
$\alpha \frak g$-currents of dimension $d$ as a subbundle
\[
\mathcal B_d^{-s} (\alpha \frak g, \Mod) := \{ \GMod (\alpha , T ) \, \, \text{
  s.t. } \, T \in \mathcal B_d (\alpha \frak g, M) \} \, \subset \, \bigwedge
{} \! ^d \alpha \frak g \otimes \Sobolev^{-s}_\alpha (\Mod)
\]
of the bundle of $\alpha \frak g$-currents of dimension $d$ and Sobolev order
$|s|$, equipped with the $\Sobolev^{-s}$-norm


\begin{proposition} \label{Lyap_renorm_inv_dist_bis} Let $s > g/2$.  The bundle
  $\mathcal B_d (\alpha \frak g, \Mod)$ of closed $\alpha \frak g$-currents of
  dimension $d$ and Sobolev order $s$ is an ``eigen-sub-bundle'' of $ \bigwedge
  ^d \alpha \frak g \otimes \Sobolev^{-s}_\alpha (\Mod)$ the renormalization
  flow $\beta_\lambda^t$, with eigenvalue $e^{\frac{d}{2}t}$. That is, for any
  $\GMod (\alpha , T)$ with $T \in \mathcal B_d (\alpha \frak g, M)$,
  \[
  \| \GMod (\alpha \beta_\lambda^t , T ) \|_{\bigwedge {} \! ^d \alpha \frak g
    \otimes \Sobolev^{-s}_\alpha (\Mod)} = e^{\frac{d}{2}t} \cdot \| \GMod
  (\alpha , T ) \|_{\bigwedge {} \! ^d \alpha \frak g \otimes
    \Sobolev^{-s}_\alpha (\Mod)} \, .
  \]
  Equivalently \cyan{(and down to Earth)}, let $D \in \mathcal D '(M) \cap
  L^2_{\neq 0}(M) $ be a distribution such that $\pi _{\alpha \frak g} (D) :=
  {}_\alpha \! X_\lambda \otimes D \in \mathcal B_d (\alpha \frak g, M) \cap
  \left( \bigwedge ^d \alpha \frak g \otimes \Sobolev^{-s}_\alpha (M) \right)$,
  i.e is a closed $\frak \alpha g$-current of dimension $d$ and Sobolev order
  $s>g/2$.  Then
  \[
  \| D \| _{\Sobolev ^{-s}_{\alpha \beta _\lambda^t}(M)} = e^{\frac{d}{2}t}
  \cdot \| D \| _{\Sobolev ^{-s}_{\alpha}(M)} \, ,
  \]
  i.e.
  \[
  \| (\alpha \beta_\lambda^t , D ) \| _{\Sobolev^{-s}(\Mod)} = e^{\frac{d}{2}t}
  \cdot \| (\alpha \beta_\lambda^t , D ) \| _{\Sobolev^{-s}(\Mod)} \, .
  \]
\end{proposition}

\paragraph{Proof.}  First, we assume we are a fixed (irreducible) Schr\"
odinger reprentation $\Sc ^\hbar$, where the space of closed distributions
(pre-images of closed currents under $\pi _{\alpha \frak g}$) is spanned by the
Schwartz distributions $I^d \times T_{\phi_a}$, for $a \in \N^{g-d}$, defined
in \eqref{closed_currents}. Then, we compute, using the Weil representation
\eqref{Weyl_representation_renormalization}
\begin{eqnarray*}
  \| I^d \times T_{\phi _a}  \| _{\Sobolev ^{-s}_{\alpha \beta _\lambda ^t}(\R^g)}   
  & = & 
  \sup _{\| \varphi  \| _{\Sobolev^s_{\alpha \beta_\lambda^t} (\R^g)} =1} \left|  \lin  I_d \times \phi_a , \varphi \rin \right|  \\
  & = & 
  \sup _{\|  (1+ {} _{\alpha \beta _\lambda^t } \! \Delta) ^{s/2} \varphi  \| _{L^2(\R^g)} =1} \left|  \int _{\R^d} \varphi (x,y)  \phi _a (y) \, dx \, dy  \right|  \\
  & = & 
  \sup _{\|  (1+ {} _{\alpha } \! \Delta) ^{s/2} \varphi  \| _{L^2(\R^g)} =1} \left|  \int _{\R^d} e^{-d/2} \varphi (e^{-t}x,y)  \phi _a (y) \, dx \, dy  \right|  \\
  & = & 
  \sup _{\|   (1+ {} _{\alpha } \! \Delta) ^{s/2}\varphi \| _{L^2(\R^g)} =1} e^{\frac{d}{2}t} \cdot \left|  \int _{\R^d} \varphi (x,y)  \phi _a (y) \, dx \, dy  \right|  \\
  & = & e^{\frac{d}{2}t} \cdot \| I_d \times T_{\phi _a}  \| _{\Sobolev ^{-s}_{\alpha }(\R^g)} 
\end{eqnarray*}
\qed


\subsection{The renormalization argument}

\paragraph{Orthogonal splittings. } Let $\lambda \in \Lambda (G,d)$, with
$1\leq d \leq g$, and $G=G_\lambda$ the corresponding coordinate type isotropic
subgroup of $\Hei$ (see subsection \ref{subsection:actions}).  In order to
simplify the notation introduced in \eqref{Sobolev_cochains} and
\eqref{Sobolev_cochains}, we set, for $s \geq 0$,
\[
\Sobolev^{s} _{\alpha ,G}:= \bigwedge {} \! ^d \alpha \frak g ^\ast \otimes
\Sobolev^{s}_\alpha (M)\qquad \text{ and }\qquad \Sobolev^{-s} _{\alpha ,G} :=
\bigwedge {} \! ^d \alpha \frak g \otimes \Sobolev^{-s}_\alpha (M)
\]
For any exponent $s>g/2$, the space $\mathcal B_d (\alpha \frak g, M)$ is a
closed subspace of the Hilbert space $\Sobolev^{-s} _{\alpha ,G} $, and
therefore induces an orthogonal decomposition
\[
\Sobolev^{-s} _{\alpha ,G} = \mathcal B^{-s} _{\alpha ,G} \oplus \mathcal
R^{-s} _{\alpha ,G} \, ,
\]
where $ \mathcal B^{-s} _{\alpha ,G} := \Sobolev^{-s}_{\alpha, G} \cap \mathcal
B_d(\alpha \frak g , M)$ and $\mathcal R^{-s} _{\alpha ,G} := \left( \mathcal
  B^{-s} _{\alpha ,G} \right) ^\perp$.  We also consider the dual orthogonal
splitting
\[
\Sobolev^{s} _{\alpha ,G}= \mathcal B^{s} _{\alpha ,G} \oplus \mathcal R^{s}
_{\alpha ,G} \, ,
\]
where $\mathcal B^{s} _{\alpha ,G} := \ker \mathcal B^{-s} _{\alpha ,G} $ and
$\mathcal R^{s} _{\alpha ,G} := \left( \ker \mathcal B^{-s} _{\alpha ,G}
\right) ^\perp$.

We use the same symbols for the subspaces and the corresponding orthogonal
projections.  Thus, if $T = \mathcal B^{-s} _{\alpha ,G} (T) + \mathcal R^{-s}
_{\alpha ,G} (T) \in \Sobolev^{-s}_{\alpha ,G}$ and $\omega = \mathcal B^{s}
_{\alpha ,G} (\omega) + \mathcal R^{s} _{\alpha ,G} (\omega) \in \Sobolev
^{s}_{\alpha ,G}$, we may write their pairing
\begin{eqnarray*}
  \lin T , \omega \rin 
  & = & 
  \lin \mathcal B^{-s} _{\alpha ,G} (T), \omega  \rin + 
  \lin \mathcal R^{-s} _{\alpha ,G} (T) , \omega  \rin \\
  & = & 
  \lin \mathcal B^{-s} _{\alpha ,G} (T), \mathcal R^{s} _{\alpha ,G} (\omega) \rin + 
  \lin \mathcal R^{-s} _{\alpha ,G} (T) , \mathcal B^{s} _{\alpha ,G} (\omega) \rin \, . 
\end{eqnarray*}
Since $\pi _{\alpha \frak g} : \mathcal D ' (M) \to \mathcal C_d(\alpha \frak g
, M)$, defined by $D \mapsto X_\lambda \otimes D$, injects distributions
(i.e. current of dimension $0$) inside currents of dimension $d$, we may also
consider the orthogonal splitting
\[
\Sobolev ^{-s} _\alpha (M) = \mathcal B ^{-s}_{\alpha , G} (M) \oplus \mathcal
R ^{-s}_{\alpha , G} (M) \, ,
\]
where $\mathcal B^{-s}_{\alpha , G } (M) = \pi_{\alpha \frak g} ^{-1} \left(
  \mathcal B^{s} _{\alpha , G} \right)$ and $\mathcal R ^{-s}_{\alpha , G} (M)
= \mathcal B^{-s}_{\alpha (\frak g)} (M) ^\perp$. For $D \in \Sobolev ^{-s}
_\alpha (M)$, we therefore denote
\[
D = \mathcal B ^{-s}_{\alpha , G} (D) + \mathcal R ^{-s}_{\alpha , G} (D)
\]
the corresponding orthogonal decomposition \cyan{(note that I'm using the same
  notation for couples of different objets: distributions and currents!)}


\paragraph{Strategy.}  We want to understand the limit of the distributions
$_\alpha G ^{T} (m)$, defined in \eqref{alternative_def_distributions}, as $T
\to \infty$, and this is the same as the limit $_\alpha G ^{e^tT} (m)$ as $t
\to \infty$. We decompose
\[
_\alpha G ^T (m) = \mathcal B _{\alpha ,G}^{-s} \left( \, _\alpha G^T (m)
\right) + \mathcal R _{\alpha ,G}^{-s} \left( \, _\alpha G^T (m) \right) \, ,
\]
then fix the Sobolev structure $\Sobolev ^s _\alpha (M)$ \cyan{(or $\Sob ^s
  _\alpha (M)$)} and try to estimate the norms
\begin{equation} \label{decomposition} \| _\alpha G ^{T} (m) \| _{\Sobolev
    ^{-s} _\alpha (M)} \leq \| \mathcal B _{\alpha,G} ^{-s} \left( _\alpha G
    ^{T} (m) \right) \| _{\Sobolev ^{-s} _\alpha (M)} + \| \mathcal R
  _{\alpha,G} ^{-s} \left( _\alpha G ^{T} (m) \right) \| _{\Sobolev ^{-s}
    _\alpha (M)}
\end{equation}
The ``rest'' $\mathcal R _{\alpha,G} ^{-s} \left( _\alpha G ^{T} (m) \right)$
will be estimated using the cohomological equation, hence reduced to a sum of
Birkhoff average of lower dimensional groups. On the other side, since, by
Lemma \ref{renormalization_covariance}, $_\alpha G ^{e^tT} = \, _{\alpha \beta
  _G^t} G ^T$, where $\beta _G^t$ is the renormalization flow adapted to the
subgroup $G$, we may define $\alpha ' = \alpha \beta _G^t$ and observe that
 
\[
\mathcal B _{\alpha,G} ^{-s} \left( _\alpha G ^{e^t T} (m) \right) = \mathcal B
_{\alpha ' \beta _G^{-t},G} ^{-s} \left( _{\alpha ' \beta _G^{-t}} G ^{e^t T}
  (m) \right) = \mathcal B _{\alpha '\beta _G^{-t},G} ^{-s} \left( _{\alpha '}
  G ^{T} (m) \right) \, .
\]
In particular,
\begin{equation} \label{trick} \| \mathcal B _{\alpha,G} ^{-s} \left( _\alpha G
    ^{e^tT} (m) \right) \| _{\Sobolev ^{-s} _\alpha (M)} = \| \mathcal B
  _{\alpha '\beta _G^{-t},G} ^{-s} \left( _{\alpha '} G ^{T} (m) \right) \|
  _{\Sobolev ^{-s} _{\alpha '\beta _G^{-t}} (M)} \, ,
\end{equation}
and it is the last expression that we will estimate using a perturbative
argument (the decomposition again) and induction on the dimension of the group
$G$.


\paragraph{Observation.} In order to shorten our formulas, from now on we won't
write explicitly the ``initial point'' $m$ in the above distributions. This is
justified a posteriori by the fact that all estimates will be uniform in $m$.

\paragraph{Estimate for the rest.}  Recall the notation introduced in
subsection \ref{subsection:actions}. The ``boundary'' $\partial G$ of the
subgroup $G=G_\lambda$ is the collection of subgroups $G_\mu$ with $\mu
\in \partial \lambda \subset \Lambda(g,d-1)$.

The solution of the cohomological equation gives

\begin{lemma} \label{rest_estimate} Let $s>g/2$. For any $u < s/g-1$, there
  exists a constant $C=C(u,s) >0$ such that
  \[
  \| \mathcal R _{\alpha,G} ^{-s} \left( \, _\alpha G ^T \right) \| _{\Sobolev
    _{\alpha} ^{-s}(M)} \leq \frac{C}{T} \cdot \sum _{F \in \partial G} \| \,
  _\alpha F ^T \| _{\Sobolev _\alpha ^{-u} (M)} \, .
  \]
  If, moreover, $G$ is $1$-dimensional and $g+1/2<u < s/g-1$ (thus
  $s>g(g+3/2)$) there exists a constant $C=C(u,s) >0$ such that
  \[
  \| \mathcal R _{\alpha,G} ^{-s} \left( \, _\alpha G ^T \right) \| _{\Sobolev
    _{\alpha} ^{-s}(M)} \leq \frac{C}{T} \cdot B_{\Sobolev^{u}}(\GMod \alpha)
  \, .
  \]
\end{lemma}

\paragraph{Proof.} 
For $G =G_\lambda \simeq \R^d$ as above, $\alpha \in \Auto$ and $m \in M$,
consider the distribution $D:= _\alpha G ^T(m)$, defined in
\eqref{alternative_def_distributions} as
\[
\lin \, D , \varphi \rin = \frac{1}{(2T)^d} \int _{|x| \leq T} \varphi ( m
\cdot \alpha \ell _{(x_1, \dots , x_d)}) \, dx_1 \dots dx_d
\]
Correspondingly, we write its orthogonal decomposition
\[
D = D_{\mathcal B}+ D_{\mathcal R} := \mathcal B _{\alpha,G} ^{-s} ( D ) +
\mathcal R _{\alpha,G} ^{-s} ( D) \, .
\]
Let $C =\pi _{\alpha \frak g} D := {}_\alpha \! X_\lambda \otimes D \in
\mathcal C_d (\alpha \frak g ,M)$ the corresponding $\alpha \frak g$-current of
dimension $d$. Clearly, its orthogonal decomposition (in the space
$\Sobolev^{-s}_{\alpha,G}$ of $\alpha \frak g$-currents of dimension $d$ and
Sobolev order $s$ !) is $C = C_{\mathcal B} + C_{\mathcal R} := {}_\alpha \!
X_\lambda \otimes D_{\mathcal B}+ {}_\alpha \! X_\lambda \otimes D_{\mathcal
  R}$.  Given a test function $\varphi \in \Sobolev ^s _\alpha (M) \cap
L^2_{\neq 0}(M)$, with $s>g/2$, let $\omega := {} _{\alpha} \! \theta_\lambda
\otimes \varphi \in \Sobolev^s_{\alpha,G}$, so that, by the definition of the
injection $\pi_{\alpha \frak g}$, we have $\lin C , \omega \rin = \lin D ,
\varphi \rin$.  Decompose $\omega = \omega _{\mathcal B} + \omega _{\mathcal R}
$ , where
\[
\omega _{\mathcal B} = {} _{\alpha} \! \theta_\lambda \otimes \varphi
_{\mathcal B } \in \ker \mathcal B_d ({\alpha \frak g} , M)
\]
and $\omega _{\mathcal R } \in \ker \left( \mathcal B_d ({\alpha \frak g} , M)
\right) ^\perp $.  But $\omega _{\mathcal B}$ is closed for dimensional reason,
and belongs to the kernel of all the closed $\alpha \frak g$-currents of
dimension $d$, therefore, by Proposition \ref{solution-cohom-eq-sobolev}, there
exists a
\[
\Omega = \sum _{\mu \in \partial \lambda}^d (-1)^k {}_\alpha \! \theta_\mu
\otimes \Omega_\mu \in \mathcal C^{d-1} (\alpha \frak g , M)
\]
which solves the cohomological equation $\D \Omega = \omega_{\mathcal B}$, so
that formally $\Omega = \D^{-1} \omega_{\mathcal B}$.  Observe that, again by
proposition \ref{solution-cohom-eq-sobolev} \cyan{(here we use the fact that we
  are in $L_{\neq 0} ^2 (M)$ !)},
\[
\| \Omega \| _{\Sobolev_\alpha ^{u} (M)} \leq C \cdot \| \omega _{\mathcal B}
\| _{\Sobolev_\alpha ^s (M)}
\]
for $u<s/g-1$ and some constant $C=C(u,s)$.  Since $\lin C_{\mathcal R} ,
\omega \rin = \lin C , \omega _{\mathcal B}\rin = \lin D , i_{{}_\alpha \!
  X_\lambda} \omega _{\mathcal B} \rin = \lin D, \varphi_{\mathcal B} \rin$,
using the cohomological equation $\D \Omega = \omega_{\mathcal B} $ (written in
coordinates!) and the definition of $D$, we see that
\begin{eqnarray*}
  \lin C_{\mathcal R} , \omega \rin & = & \frac {1}{(2T)^d}  \int _{|x|_\infty \leq T} \sum _{k=1}^d \left( \partial _{_\alpha X_k} \psi _k \right) (m \cdot \alpha \ell _{(x_1,\dots , x_d)} ) dx_1 \dots dx_d \, , 
\end{eqnarray*}
where the $\psi _k$'s are the coordinates $\Omega _{\mu}$'s, since the $\mu
\in \partial \lambda$ may be indexed by $k=1,\dots, d$.  Integrating each
addend above w.r.t. the correspondent variable $x_k$ from $-T$ to $T$, we
finally get
\begin{eqnarray*}
  \lin C_{\mathcal R} , \omega \rin & = & \frac {1}{2T} \sum_{j= \pm 1}  \sum _{k=1}^d \frac{j}{(2T)^{d-1}} \int _{|x|_\infty \leq T}  \psi _k (m \cdot \alpha \ell _{(x_1,\dots , j T, \dots x_d)} ) dx_1 \dots \check{dx_k} \dots dx_d \\
  & = & 
  \frac{1}{2T} \cdot \sum_{j= \pm 1} \sum _{F \in \partial G}   \lin  \, _\alpha F^T (m \cdot \alpha \ell _{(0, \dots , j T, \dots , 0)} ) , \psi_k \rin 
\end{eqnarray*}
For $d \geq 2$, we may further estimate
\begin{eqnarray*}
  | \lin C_{\mathcal R} , \omega \rin | & \leq & 
  \frac{1}{T} \cdot \sum _{F \in \partial G}  \left| \lin  \, _\alpha F^T (m \cdot \alpha \ell _{(0, \dots , \pm T, \dots , 0)} ) , \phi_k \rin \right| \\ 
  & \leq & 
  \frac{1}{T} \cdot \sum _{F \in \partial G}  \| _\alpha F^T (m \cdot \alpha \ell _{(0, \dots , \pm T, \dots , 0)} ) \| _{\Sobolev ^{-u}_\alpha (M)} \cdot \| \phi_k \| _{\Sobolev^{u}_\alpha (M) } \\
  & \leq & 
  \left( \frac{C}{T} \cdot \sum _{F \in \partial G} \| _\alpha F^T (m \cdot \alpha \ell _{(0, \dots , \pm T, \dots , 0)} ) \| _{\Sobolev ^{-u}_\alpha (M)} \right) \cdot \| \varphi \| _{\Sobolev^s_\alpha (M) }
\end{eqnarray*}
if $u< s/g-1$, which is what we wanted to prove. For $d=1$, we simply observe
that
\begin{eqnarray*}
  | \lin C_{\mathcal R} , \omega \rin | & \leq & 
  \frac{C}{T} \cdot \| \Omega \|_{\infty}  \\ 
  & \leq & \frac{C}{T} \cdot B_{\Sobolev^{u}} (\GMod \alpha ) \cdot \| \Omega  \|_{\Sobolev_\alpha^{u}(M)} \\
  & \leq & \frac{C}{T} \cdot B_{\Sobolev^{u}} (\GMod \alpha ) \cdot \| \omega \|_{\Sobolev_\alpha^{s}(M)} 
\end{eqnarray*}
\qed





\paragraph{Perturbative argument for the dominant part.}  \cyan{``a
  sufficiently small perturbation of a contraction is still a contraction''}

For any $t \in \R$, we consider the decomposition
\[
_\alpha G ^T = \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T
\right) + \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T
\right) \, ,
\]
For any $ \tau \in \R$, we use the above decomposition to write
\begin{eqnarray*}
  \mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s}  \left( _\alpha G ^T \right) 
  & = & 
  \mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s}  \left( \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T  \right) \right) 
  + \mathcal B _{\alpha \beta _G^{-(t+\tau) },G} ^{-s}  \left( \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right) \right)  \\
  & = & 
  \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right)  
  + \mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s}  \left( \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right) \right)
\end{eqnarray*} 
(we used the fact that $\mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s} =
\mathcal B _{\alpha \beta _G^{-t},G} ^{-s}$ for any $t,\tau \in \R$).  Now we
compute the norm in $\Sobolev^s_{\alpha \beta _G^{-(t+\tau)}} (M)$ (but we
suppress the $M$'s from the notation!), use Proposition
\ref{Lyap_renorm_inv_dist_bis} and the fact that the $\mathcal B$'s are a
projections, to estimate
\begin{eqnarray*}
  \| \mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s}  \left( _\alpha G ^T  \right) \| _{\Sobolev^{-s}_{\alpha \beta _G^{-(t+\tau)}} } 
  & \leq & 
  \| \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} ( \, _\alpha G^T  )  \| _{\Sobolev^{-s}_{\alpha \beta _G^{-(t+\tau)}} } 
  + \| \mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s}  \left( \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} ( \, _\alpha G^T ) \right)
  \| _{\Sobolev^{-s}_{\alpha \beta _G^{-(t+\tau)}} } \\
  & \leq & 
  e^{-\frac{d}{2} \tau} \cdot \| \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T  \right)  \| _{\Sobolev^{-s}_{\alpha \beta_G^{-t}} } 
  + \|  \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right) \| _{\Sobolev^{-s}_{\alpha \beta _G^{-(t-\tau)}} }
\end{eqnarray*}
We fix the ``step'' $\tau>0$.  We claim that an analogue of Lemma 3.9 of
\cite{MR2218767} holds\marginpar{\cyan{TRUE?}}, actually that as long as $\tau$
is bounded, the norms $\| \cdot \|_{\Sobolev^{-s}_{\alpha \beta _G^{\tau}}}$
and $\| \cdot \|_{\Sobolev^{-s}_{\alpha} }$ are within a bounded ratio.

There follows that there exists a constant $C=C(G, s,\tau) >0$ such that
\begin{eqnarray*}
  \| \mathcal B _{\alpha \beta _G^{-(t+\tau)},G} ^{-s}  \left( _\alpha G ^T  \right) \| _{\Sobolev^{-s}_{\alpha \beta _G^{-(t+\tau)}} } 
  & \leq &  
  e^{-\frac{d}{2} \tau} \cdot \| \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T  \right)  \| _{\Sobolev^{-s}_{\alpha \beta_G^{-t}} } 
  + C \cdot  \|  \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right) \| _{\Sobolev^{-s}_{\alpha \beta _G^{-t}} } 
\end{eqnarray*}
which, using Lemma \ref{renormalization_covariance}, may be rewritten in the
convenient form
\begin{eqnarray*} \label{perturbative_first_step} \| \mathcal B _{\alpha \beta
    _G^{-(t+\tau)},G} ^{-s} \left( _\alpha G ^T \right) \|
  _{\Sobolev^{-s}_{\alpha \beta _G^{-(t+\tau)}} } & \leq & e^{-\frac{d}{2}
    \tau} \cdot \| \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha
    G^T \right) \| _{\Sobolev^{-s}_{\alpha \beta_G^{-t}} } + C \cdot \|
  \mathcal R _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _{\alpha \beta _G^{-t}}
    G^{e^\tau T} \right) \| _{\Sobolev^{-s}_{\alpha \beta _G^{-t}} }
\end{eqnarray*}
We set $ t = n \tau$ for integer $n \in \N$. Then, the above is a recursive
inequality
\begin{equation} \label{recursive_ineq} X_{n+1} \leq e^{-\frac{d}{2}\tau} \cdot
  X_n + C \cdot R_k
\end{equation}
for the norms
\begin{equation} \label{boundary} X_n := \| \mathcal B _{\alpha \beta
    _G^{-n\tau},G} ^{-s} \left( \, _\alpha G^T \right) \|
  _{\Sobolev^{-s}_{\alpha \beta_G^{-n\tau}} }
\end{equation}
that we are trying to estimate, depending on the ``parameters''
\begin{equation} \label{rest} R_n:= \left\| \mathcal R _{\alpha \beta
      _G^{-n\tau},G} ^{-s} \left( \, _{\alpha \beta _G^{-n\tau}} G^{e^{k\tau}
        T} \right) \right\| _{\Sobolev^{-s}_{\alpha \beta _G^{-n \tau}} } \, .
\end{equation}
The solution of the recursive inequality \eqref{recursive_ineq} is
\begin{equation} \label{solution_rec_ineq} X_{n} \leq e^{-\frac{d}{2} n\tau }
  \left( X_0 + C \cdot e^{\frac{d}{2}\tau} \cdot \sum_{k=0}^{n-1}
    e^{\frac{d}{2} k \tau } \cdot R_k \right)
\end{equation}

Now, we start with the $1$-dimensional case.

\begin{lemma} \label{perturbative_one_dim} Let $G$ be a $1$-dimensional
  (isotropic) subgroup of $\Hei$, and $s>g(g+3/2)$. Assume that the point
  $\GMod \alpha \in \Mod$ is such that there exist $\varepsilon >0$ and $C>0$
  such that
  \[
  \left( \det Y(\GMod \alpha \beta_G^{- t}) \right)^{1/4} \leq C \cdot
  e^{\left( \frac{1}{2}-\varepsilon \right)t} \qquad \qquad \forall t>0 \, .
  \]
  For example this is true if $\GMod \alpha$ is of bounded type, if it
  satisfies a Roth condition, or if it is Diophantine of any type $\sigma > 0
  $. Then for all $T \gg 1$
  \[
  \| \mathcal B _{\alpha ,G} ^{-s} \left( \, _\alpha G^{T} \right) \|
  _{\Sobolev^{-s}_{\alpha} } \leq \frac{C}{T^{1/2}} \cdot B_{\Sob^s} \left(
    \GMod \alpha \beta_G^{\log T} \right) \, .
  \]
\end{lemma}

\paragraph{Proof. } According to lemma \ref{rest_estimate}, we may estimate the
rest, as defined in \eqref{rest}, as
\begin{equation} \label{R_k} R_n = \| \mathcal R _{\alpha \beta _G^{-n\tau},G}
  ^{-s} \left( \, _{\alpha \beta _G^{-n\tau}} G^{e^{n\tau} T} \right) \|
  _{\Sobolev^{-s}_{\alpha \beta _G^{-n \tau}} } \leq \frac{C}{e^{n\tau} T}
  \cdot B_{\Sobolev^{u}} (\GMod \alpha \beta_G^{-n \tau} )
\end{equation}
provided $g+1/2<u<s/g-1$. Therefore, using Proposition
\ref{best_Sobolev_constant} and the hypothesis, we have the bound
\[
R_n \leq \frac{C}{e^{n\tau} T} \cdot \left( \det Y (\GMod \alpha
  \beta_G^{-n\tau} \right) ^{1/4} \leq \frac{C}{e^{n\tau} T} \cdot e^{\left(
    \frac{1}{2}-\varepsilon \right)nt} \leq \frac{C}{T} \cdot e^{\left(
    -\frac{1}{2}-\varepsilon \right)nt} \, .
\]
There follows that the solution \eqref{solution_rec_ineq} of the recursive
inequality \eqref{recursive_ineq} is bounded by
\begin{eqnarray*}
  X_{n} & \leq & e^{-\frac{1}{2} n \tau } \left( X_0 +\frac{C}{T}
    e^{\frac{1}{2}\tau} \cdot \sum_{k=0}^{n-1} e^{\frac{1}{2} k \tau }  e^{\left( -\frac{1}{2}-\varepsilon \right)kt} \right) \\
  & \leq & e^{-\frac{1}{2} n \tau } \left( X_0 + \frac{C}{T} \right) \, . 
\end{eqnarray*}
\cyan{(the point is that we get a bound $ X_n \sim e^{\frac{1}{2} n \tau} X_0$
  provided we may bound the sum $\sum _{k=0}^{n-1} e^{\frac{1}{2} k \tau }
  \cdot R_k $. This happens when $\alpha$ is of bounded type, or Diophantine of
  any type $\sigma >0$ (see \eqref{Diophantine_best_Sobolev_constant})} Going
back to our previous notation, and setting $t = n \tau$, the above inequality
says that
\[
\| \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right) \|
_{\Sobolev^{-s}_{\alpha \beta_G^{-t}} } \leq e^{-\frac{1}{2} t } \left( \|
  \mathcal B _{\alpha,G} ^{-s} \left( \, _\alpha G^T \right) \|
  _{\Sobolev^{-s}_{\alpha} } + \frac{C}{T} \right) \, .
\]
Now we use \eqref{trick} and estimate
\begin{eqnarray*}
  \| \mathcal B _{\alpha ,G} ^{-s} \left( \, _\alpha G^{e^tT} \right)  \| _{\Sobolev^{-s}_{\alpha} }
  & = & 
  \| \mathcal B _{(\alpha \beta_G^t) \beta _G^{-t},G} ^{-s} \left( \, _{\alpha \beta_G^t}G^T \right)  \| _{\Sobolev^{-s}_{(\alpha \beta_G^t) \beta_G^{-t}} } \\
  & \leq & 
  e^{-\frac{1}{2} t } 
  \left( \| \mathcal B _{\alpha \beta_G^t ,G} ^{-s} \left( \, _{\alpha \beta_G^t}G^T \right)  \| _{\Sobolev^{-s}_{\alpha \beta_G^t} } + \frac{C}{T} \right) \\
  & \leq & 
  e^{-\frac{1}{2} t } 
  \left( B_{\Sobolev^s} \left( \GMod \alpha \beta_G^t \right)  + \frac{C}{T} \right) 
  \qquad \qquad \text{ (by lemma \ref{trivial_bound_Sobolev})}
\end{eqnarray*}
The lemma follows if we take first $T=1$ and then rename $e^t := T \gg 1$.
\qed

\bigskip

Combining Lemmas \ref{rest_estimate} and \ref{perturbative_one_dim}, and once
again Proposition \ref{best_Sobolev_constant}, we see that the norm of the
Birkhoff averages for the action of a $1$-dimensional isotropic subgroup $G
\subset \Hei$ are bounded by
\begin{eqnarray*}
  \| _\alpha G ^T \| _{\Sobolev_\alpha ^{-s}(M)} 
  & \leq &  
  \frac{C}{T^{1/2}} \cdot B_{\Sobolev^s} \left( \GMod \alpha \beta_G^{\log T} \right) \\
  & \leq & 
  \frac{C}{T^{1/2}} \cdot  \left( Y(\GMod \alpha \beta_G^{\log T} \right)^{1/4} \, , 
\end{eqnarray*}
provided $s > g(g+3/2)$, thus depend on the ``escape rate'' of (the projection
of) the point $\GMod \alpha \beta_G^t $ into the cusp of the Siegel modular
variety. We record the possible asymptotics in the following

\begin{proposition} \label{equidistribution_one_dim} Let $G$ be a
  $1$-dimensional (isotropic) subgroup of $\Hei$, and let $s>g(g+3/2)$.
  \begin{itemize}
  \item If $\GMod \alpha$ is of bounded type, then there exists a constant
    $C>0$ such that
    \[ \left| \lin _\alpha G ^T , \varphi \rin \right| \leq \frac{C}{T^{1/2}}
    \cdot \| \varphi \| _{\Sobolev^s_\alpha (M)} \, , \]
  \item if $\GMod \alpha$ satisfies a Roth condition, then for any $\varepsilon
    >0$ there exists a constant $C>0$ such that
    \[ \left| \lin _\alpha G ^T , \varphi \rin \right| \leq
    \frac{C}{T^{1/2-\varepsilon}} \cdot \| \varphi \| _{\Sobolev^s_\alpha (M)}
    \, , \]
  \item if $\GMod \alpha$ is Diophantine of type $\sigma >0$, then there exists
    a constant $C>0$ such that
    \[ \left| \lin _\alpha G ^T , \varphi \rin \right| \leq
    \frac{C}{T^{\sigma/2}} \cdot \| \varphi \| _{\Sobolev^s_\alpha (M)} \, , \]
  \end{itemize}
  for all $T \gg 1$ and all test functions $\varphi \in \Sobolev^s _\alpha (M)
  \cap L_{\neq 0} ^2(M)$.
\end{proposition}

Moreover, it follows from the Kleinbock-Margulis logarithm law, via Proposition
\ref{Sobolev_constant_estimate}, that

\begin{proposition} \label{equidistribution_one_dim_KM} Let $G$ be a
  $1$-dimensional (isotropic) subgroup of $\Hei$, and let $s>g(g+3/2)$.  There
  exists a full measure set $\Omega_g \subset \Sigma_g$ inside the Siegel
  modular variety such that if $\GMod \alpha \in \Mod$ projects to $\Omega_g$
  then
  \[
  \left| \lin _\alpha G ^T , \varphi \rin \right| \leq C \cdot \frac{( \log T)
    ^{\frac{g+1}{8}}}{T^{1/2}} \cdot \| \varphi \| _{\Sobolev^s_\alpha (M)}
  \]
  for all $T \gg 1$ and all test functions $\varphi \in \Sobolev^s _\alpha (M)
  \cap L_{\neq 0} ^2(M)$.
\end{proposition}

Now we may use induction on the dimension of the isotropic group $G \subset
\Hei$, at least for those $\GMod \alpha$'s satisfying a Roth condition (for
example of bounded type). Let $(s_d)_{d\in \N}$ be the solution of the
recursive equation $s_{d+1} = g(s_d+1)$ with initial condition $s_1 =
g(g+3/2)$. \cyan{(observe that $s_d \approx g^{d+1}$)}

\begin{proposition} \label{equidistribution_d_dim_Roth} Let $G$ be a isotropic
  subgroup of $\Hei$ of dimension $1\leq d \leq g$, and let $s>s_d$.
  \begin{itemize}
  \item If $\GMod \alpha \in \Mod$ satisfies a Roth condition (for example,
    $\GMod \alpha$ projects to the full measure set $\Omega_g\subset \Sigma_g$
    appearing in the Kleinbock-Margulis logarithmic law), then for any
    $\varepsilon >0$ there exists a constant $C=C(G,\alpha,s,g, \varepsilon)>0$
    such that
    \[ \left| \lin _\alpha G ^T , \varphi \rin \right| \leq
    \frac{C}{T^{\frac{d}{2}-\varepsilon}} \cdot \| \varphi \|
    _{\Sobolev^s_\alpha (M)} \, ,
    \]
  \item if $\GMod \alpha \in \Mod$ is of bounded type, then there exists a
    constant $C=C(G,\alpha,s,g)>0$ such that
    \[
    \left| \lin _\alpha G ^T , \varphi \rin \right| \leq
    \frac{C}{T^{\frac{d}{2}}} \cdot \| \varphi \| _{\Sobolev^s_\alpha (M)}
    \]
  \end{itemize}
  for all $T \gg 1$ and all test functions $\varphi \in \Sobolev^s _\alpha (M)
  \cap L_{\neq 0} ^2(M)$.
\end{proposition}
.

\paragraph{Proof.} We argue by induction. The case $d=1$ has already been
proven in Proposition \ref{equidistribution_one_dim}. We assume the result
holds for $d-1 \geq 1$, and use the notation introduced in \eqref{boundary} and
\eqref{rest}. According to Lemma \ref{rest_estimate}, we may estimate
\begin{equation} \label{R_k} R_n = \| \mathcal R _{\alpha \beta _G^{-n\tau},G}
  ^{-s} \left( \, _{\alpha \beta _G^{-n\tau}} G^{e^{n\tau} T} \right) \|
  _{\Sobolev^{-s}_{\alpha \beta _G^{-n \tau}} } \leq \frac{C}{e^{n \tau} T}
  \cdot \sum _{F \in \partial G} \| \, _\alpha F ^{e^{ n\tau}T} \| _{\Sobolev
    _\alpha ^{-u}}
\end{equation}
provided $u<s/g-1$. By the inductive hypothesis,
\[
\| \, _\alpha F ^{e^{n \tau}T} \| _{\Sob _\alpha ^{-u}} \leq \frac{C}{(e^{
    n\tau}T)^{\frac{d-1}{2}-\varepsilon}}
\]
and consequently
\[
R_n \leq \frac{C}{e^{ n\tau} T} \cdot \frac{C}{(e^{
    n\tau}T)^{\frac{d-1}{2}-\varepsilon}} \leq
\frac{C}{T^{\frac{d+1}{2}-\varepsilon}} \cdot e^{-(\frac{d+1}{2}-\varepsilon)
  n\tau}
\]
for any $\varepsilon >0$ in the Roth case, and for $\varepsilon =0$ in the
bounded type case, as long as $u>s_{d-1}$ (therefore $s > g(u+1) \geq
s_d$). There follows that the solution \eqref{solution_rec_ineq} of the
recursive inequality \eqref{recursive_ineq} is bounded by
\begin{eqnarray*}
  X_{n} 
  & \leq & e^{-\frac{d}{2} n \tau } \left( X_0 + C \cdot e^{\frac{d}{2}\tau} \cdot \sum_{k=0}^{n-1} e^{\frac{d}{2} k \tau } \cdot R_k \right) \\
  & \leq & 
  e^{-\frac{d}{2} n\tau } \left( X_0 +  \frac{C}{T^{\frac{d+1}{2}-\varepsilon}}\cdot e^{\frac{d}{2}\tau} \cdot \sum_{k=0}^{n-1} e^{\frac{d}{2} k \tau } \cdot e^{-(\frac{d+1}{2}-\varepsilon)k \tau} \right) \\
  & \leq & 
  e^{-\frac{d}{2} n\tau } \left( X_0 +  \frac{C}{T^{\frac{d}{2}}} \right) 
\end{eqnarray*}
(the sum converges even for $\varepsilon =0$).  As in the proof of the
$1$-dimensional case, and setting $t = n\tau$, this gives
\[
\| \mathcal B _{\alpha \beta _G^{-t},G} ^{-s} \left( \, _\alpha G^T \right) \|
_{\Sobolev^{-s}_{\alpha \beta_G^{-t}} } \leq e^{-\frac{d}{2} t } \left( \|
  \mathcal B _{\alpha,G} ^{-s} \left( \, _\alpha G^T \right) \|
  _{\Sobolev^{-s}_{\alpha} } + \frac{C}{T^{\frac{d}{2}}} \right)
\]
Now we use \eqref{trick} and estimate
\begin{eqnarray*}
  \| \mathcal B _{\alpha ,G} ^{-s} \left( \, _\alpha G^{e^tT} \right)  \| _{\Sobolev^{-s}_{\alpha} }
  & = & 
  \| \mathcal B _{(\alpha \beta_G^t) \beta _G^{-t},G} ^{-s} \left( \, _{\alpha \beta_G^t}G^T \right)  \| _{\Sobolev^{-s}_{(\alpha \beta_G^t) \beta_G^{-t}} } \\
  & \leq & 
  e^{-\frac{d}{2} t } 
  \left( \| \mathcal B _{\alpha \beta_G^t ,G} ^{-s} \left( \, _{\alpha \beta_G^t}G^T \right)  \| _{\Sob^{-s}_{\alpha \beta_G^t} } + \frac{C}{T^{\frac{d}{2}}} \right) \\
  & \leq & 
  e^{-\frac{d}{2} t } 
  \left( B_{\Sobolev^s} \left( \GMod \alpha \beta_G^t \right)  + \frac{C}{T^{\frac{d}{2}}} \right) 
  \qquad \qquad \text{ (by lemma \ref{trivial_bound_Sobolev})}
\end{eqnarray*}
If we first take $T=1$, and then rename $e^t = T \gg 1$, we get
\begin{equation} \label{main_term_d_dim} \| \mathcal B _{\alpha ,G} ^{-s}
  \left( \, _\alpha G^{T} \right) \| _{\Sobolev^{-s}_{\alpha} } \leq
  \frac{C}{T^{d/2}} \cdot B_{\Sobolev^s} \left( \GMod \alpha \beta_G^{\log T}
  \right) \, ,
\end{equation}
for $T \gg 1$. Combining \eqref{main_term_d_dim} with Lemma
\ref{rest_estimate}, together with the inductive hypothesis and Proposition
\ref{best_Sobolev_constant}, we see that the norm of the Birkhoff averages are
bounded by
\begin{eqnarray*}
  \| _\alpha G ^T \| _{\Sobolev_\alpha ^{-s}} 
  & \leq & 
  \frac{C}{T^{d/2}} \cdot  \left( Y \left( \GMod \alpha \beta_G^{\log T} \right) \right)^{1/4} \, . 
\end{eqnarray*}
The result follows from the bounded type \eqref{bounded_type} or the Roth
condition \eqref{Roth} on $\GMod \alpha$.  \qed


\subsection{Birkhoff averages and Theta sums}

~\cite{MR0414785, MR0466409, MR487050, MR2218767}

Here we consider the standard lattice $\Gamma = \Z^g \times \Z^g \times \{ 1
\}$ of the reduced Heisenberg group and the standard nilmanifold $M = \Gamma
\backslash \Hei$.

\paragraph{First return map.} 
The subgroup $N = \{(0, \xi , z ) \, \text{with } \, \xi \in (\R^n)^\ast \, ,
\, z \in \T \}$ is a normal subgroup of $\Hei$. The quotient $N \backslash
\Hei$ is isomorphic to the Lagrangian subgroup $ L = \{ (x, 0, 1) \, \text{with
}\, x \in \R^g \}$, and we have an exact sequence $ 0 \rightarrow N \rightarrow
\Heis \rightarrow L \rightarrow 0$.  Therefore $\Heis \simeq N \rtimes L$, and
in particular any $(x, \xi , z) \in \Hei$ may be uniquely written as the
product of an element of $N$ times an element of $H$, namely
\[
(x, \xi , t ) = (0, \xi , z ) \cdot (x, 0, 1) \, .
\]
Fix an automorphism $\alpha =(S,y,\eta) \in \Auto $, so that (see
\eqref{monomorphism} and \eqref{def_f})
\[
\alpha L = \{ \alpha \ell _x := (Ax, Cx, \lin 2^{-1} A^tCx + \eta , x \rin ) \,
\text{with }\, x \in \R^g \}\, .
\]
If $A\in \Aut (\R^g)$, i.e. if $A$ is invertible, then any element of $\Hei$
can still be written uniquely as a product
\begin{eqnarray*}
  (0,\xi, z) \cdot \alpha \ell _x & = & (0, \xi , z) \cdot (Ax, Cx, \lin  2^{-1} A^tCx + \eta , x\rin ) \\
  & = & (Ax, \xi + Cx, z \cdot  \lin  2^{-1} A^tCx + \eta , x\rin )
\end{eqnarray*}
for some $x \in \R^g$, $\xi \in (\R^g)^\ast$ an $z \in \T$.  Observe that,
given $n \in \Z^g$ and $m \in \Z^g$, i.e.  $(n,m,1) \in \Gamma$, then
\begin{equation} \label{first_return_map} (n,m,1) \cdot (0,\xi, z ) \cdot
  \alpha \ell _x = (0,\xi _{n,m}, z _{n,m}) \cdot \alpha \ell_{x _{n,m}})
\end{equation}
if and only if
\begin{eqnarray*}
  x_{n,m} & = & x+A^{-1} n\\
  \xi _{n,m} & = &  \xi + m - CA^{-1} n \\ 
  z_{n,m} & = & z \cdot \lin A^t \xi -\eta - 2^{-1}A^t CA^{-1} n, A^{-1} n \rin 
\end{eqnarray*}
(here you must use the fact that $A^tC$ is symmetric!).
  
\paragraph{Birkhoff averages of certain functions on the circle.} Let $\varphi
\in \SB ( \T)$, and let $\psi \in \mathcal E (\R^g)$ be a smooth function with
compact support.  Define a function $\phi : \Hei \to \CC$ as the product
\[
\phi ( (0, \xi , z ) \cdot \alpha \ell _x ) = \psi (x) \cdot \varphi (z)
\]
(observe that it does not depend on the $\xi$ variable, therefore its support,
if it is not empty, is not compact!).  ``Extend'' $\phi$ to a
$\Gamma$-invariant function on $\Hei$, therefore a function $\Phi :M \to \CC$
on the quotient, summing over the lattice $\Gamma $, namely
\begin{eqnarray*}
  \Phi (\Gamma \cdot (0,\xi, z) \cdot \alpha \ell_x ) & :  = & \sum _{(n,m) \in \Z^g \times \Z^g}  \phi  ( (n,m,1) \cdot (0, \xi , z ) \cdot \alpha \ell _x)  \\
  & = & \sum _{(n,m) \in \Z^g \times \Z^g}  \phi \left( (0,\xi _{n,m}, z _{n,m}) \cdot \alpha \ell _{x _{n,m}}) \right) \qquad \text{(using \eqref{first_return_map})}\\
  & = & \sum _{n \in \Z^g}  \psi \left( x+A^{-1} n \right) \cdot  \varphi \left( z \cdot  \lin A^t \xi -\eta - 2^{-1}A^t CA^{-1}n, A^{-1}n \rin\right) 
\end{eqnarray*}
Since $\psi$ has compact support, this sum is finite for all points $\Gamma
\cdot (0,\xi,z) \cdot \alpha \ell_x) \in M$, and $\Phi$ is (projects to) indeed
a smooth function on $M$.

Let $m = \Gamma \cdot (0,\xi, z ) \cdot \alpha \ell _x \in M$ be a point in the
Heisenberg homogeneous space, and let $U \subset \R^g$ be a measurable subset
with finite and positive mass. Then, we may compute the Birkhoff average of
$\Phi$ along the $\alpha L$-orbit through $m$ as follows:
\begin{eqnarray*}
  \lin \, _\alpha L ^U (m) , \Phi \rin & = & \frac{1}{|U|} \cdot \int _{U} \Phi (m \cdot \alpha \ell _y ) \, d y \\
  & = & \frac{1}{|U|} \cdot \int _{U} \Phi (\Gamma \cdot (0, \xi, z) \cdot \alpha \ell _x \cdot \alpha \ell _{y}   ) \, dy \\
  & = & \frac{1}{|U|} \cdot \int _{U} \Phi (\Gamma \cdot (0, \xi, z) \cdot \alpha \ell _{x+y}   ) \, dy \\
  & = & \frac{1}{|U|} \cdot \int _{U} \left( \sum _{a \in \Z^n }  \psi  (y+x+A^{-1}a ) \cdot \varphi \left( z \cdot \lin A^t \xi -\eta - 2^{-1}A^t CA^{-1}a, A^{-1}a \rin \right)  \right) \, dy \\
  & = & \frac{1}{|U|} \sum _{n \in \Z^g } \left( \varphi \left( z \cdot \lin A^t \xi -\eta - 2^{-1}A^t CA^{-1}n, A^{-1}n \rin\right)  \cdot \int _U \psi  (y+x+A^{-1} n ) \, dy \right) \, . 
\end{eqnarray*}
Now, we claim that, given a compact not too wild $U\subset \R^g$, it is
possible to choose a function $\psi$ in such a way that the above integral over
$U$ splits as the sum on a finite number of integrals of equal mass, one for
each lattice point $n \in \Z^g$ such that $x + A^{-1} n\in U$.  This would give
something like a ``theta sum''.

Indeed, let $\delta = \min _{n \in \Z^g \backslash \{0 \}} |A^{-1}n| >0$ (since
$A$ is invertible!).  Choose $\psi \in \mathcal E (\R^g)$ with support in a
small ball $B_\varepsilon (0) = \{x \in \R^g \, \, \text{s.t. }\, |x|_\infty
\leq \varepsilon \}$, for some $0<\varepsilon <\delta /2$, and unit mass $\int
_{\R^g} \psi (x) dx = 1$.  Choose $U$ in such a way that if $ A^{-1} n \in U$
for some $n \in \Z^g$, then the whole $\varepsilon$-neighborhood of $A^{-1}n$
belongs to $U$. For example, given any value $R=|A^{-1}n|$, for integer $n \in
\Z^g$, we may take for $U$ the ball (well, ``box'', since we are using the $|
\cdot |_\infty$ norm!) of radius $R+\delta/2$ around the origin.  For $x=0$,
$\xi =0$ and $z=1$, we get
\begin{equation} \label{Birkhoff_sums_theta} \lin \, _\alpha \! L ^U (m) , \Phi
  \rin = \frac{1}{|U|} \sum_{n \in \Z^g \, , \, \, A^{-1}n \in U} \varphi
  \left( e^{-\pi i X n\cdot n -2\pi i y \cdot n} \right)
\end{equation}
where $X$ is the symmetric operator $X :=CA^{-1}$, and $y = (A^{-1})^t \eta $.

There follows from Proposition \ref{equidistribution_d_dim_Roth} and the above
discussion (i.e. formula \ref{Birkhoff_sums_theta}) that

\begin{proposition}\label{pretheta_sums_bad} 
  Let $\alpha \in \Auto$ be an automorphism of $\Hei$ which induces the
  symplectic map $S = \left( \begin{array}{cc} A & B \\ C & D \end{array}
  \right) \subset \Symp_{2g}(\R)$ on the quotient $\Hei / \T$, define $X
  :=CA^{-1}$, and let $p \in \R^g$. For any test function $\varphi \in \Sobolev
  ^s(\T)$ with Sobolev order/exponent $s$ large enough (actually $s>s_g \approx
  g^{g+1}$), for example $\varphi \in C^\infty (\T)$, and zero average $
  \int_0^1\varphi (e^{2\pi i t} ) \, dt=0$, we have the following:

  \begin{itemize}
  \item if $\GMod \alpha$ satisfies a Roth condition (for example, projects to
    the full measure set $\Omega_g \subset \Sigma_g$ appearing in the
    Kleinbock-Margulis logarithm law) then for any $\varepsilon >0$
    \[
    \sum _{n \in \Z^g \, , \, |A^{-1}n| \leq N} \varphi \left( e^{\pi i X n
        \cdot n + 2\pi i p \cdot n} \right) = \mathcal O \left(
      N^{\frac{g}{2}-\varepsilon} \right) \qquad \text{ as } \, N \to \infty \,
    ,
    \]
  \item if $\GMod \alpha$ is of bounded type, then
    \[
    \sum _{n \in \Z^g \, , \, |A^{-1}n| \leq N} \varphi \left( e^{\pi i X n
        \cdot n + 2\pi i p \cdot n} \right) = \mathcal O \left( N^{\frac{g}{2}}
    \right) \qquad \text{ as } \, N \to \infty \, .
    \]
  \end{itemize}
\end{proposition}



\paragraph{Riemann-Siegel theta function and sums.} Gaussians are exponentials
of quadratic forms. A generic quadratic polynomial with complex coefficients on
$\R^g$ may be written as
\[
Q(x) = \pi i Zx \cdot x + 2\pi i z \cdot x + c
\]
where $Z=X+iY\in \Sym _g(\CC)$ is a symmetric $n\times n$ complex matrix
defining the quadratic form $Z[x]=Zx \cdot x$, $ z \in \CC^g$ and $c \in \CC$.
The exponential $e^{Q(x)}$ is in the space $\SB '(\R^g)$ of tempered
distributions if $Y \geq 0$. It is in the Schwartz space $\SB (\R^g)$ iff
$Y>0$, i.e. if $Z \in \Siegel _g$, and such functions $G(x)=e^{Q(x)}$ are then
called \emph{Gaussians}. The sum of the series
\[
\Theta (Z \, ; z) := \sum_{ n \in \Z ^g} e^{Q(n)} = \sum_{ n \in \Z ^g} e^{
  i\pi \, Z n \cdot n +i2\pi \, z \cdot n }\, ,
\]
defined for $Z \in \Siegel _g$ and $z\in \CC ^g$, is the \emph{Riemann-Siegel
  theta function} (~\cite{MR2352717, MR2307769}).  It reduces to the Jacobi
theta function for $g=1$.  We define the \emph{Riemann-Siegel theta sums} (or
\emph{multidimensional Gaussian exponential sum}, \cyan{or what?})  as
\[
\sum _{n \in \Z^g \, , \, |n| \leq N} e^{i\pi Xn \cdot n + i2\pi p \cdot n} \,
,
\]
for $X \in \Sym _g(\R)$ and $p \in \R^g$.  It may be thought as boundary values
(values for $Z = X + iY$ with $Y=0$) of the Riemann-Siegel theta functions.
  
If we take $\varphi (z) = z$ in Proposition \ref{pretheta_sums_bad}, we get

\begin{proposition}\label{theta_sums_bad} 
  Let $\alpha$, $X$ and $p$ as in Proposition \ref{pretheta_sums_bad}.
  \begin{itemize}
  \item if $\GMod \alpha$ satisfies a Roth condition, then for any $\varepsilon
    >0$.
    \[
    \sum _{n \in \Z^g \, , \, |A^{-1}n| \leq N} e^{\pi i Xn \cdot n + 2\pi i p
      \cdot n} = \mathcal O \left( N^{\frac{g}{2}-\varepsilon} \right) \qquad
    \text{ as } \, N \to \infty \, ,
    \]
  \item if $\GMod \alpha$ is of bounded type, then
    \[
    \sum _{n \in \Z^g \, , \, |A^{-1}n| \leq N} e^{\pi i Xn \cdot n + 2\pi i p
      \cdot n} = \mathcal O \left( N^{\frac{g}{2}} \right) \qquad \text{ as }
    \, N \to \infty \, .
    \]
  \end{itemize}
\end{proposition}

\paragraph{Heuristics.} Observe that we are summing $\sim N^g$ terms of order
one, so the trivial bound is $\mathcal O (N^g)$. If the different values
$Q(n):= \pi Xn \cdot n + 2 \pi p \cdot n $ of the quadratic form were
uncorrelated ``angles'' (as seen in the circle $\R / 2\pi \Z$), namely
independent and uniform in $[0,1]$, hence their imaginary exponentials $e^{ i
  Q(n)}$ look like steps of a random walk in the plane, we could expect a sum
of order $\mathcal O ( \sqrt{N^g})$.

\bigskip
\begin{center}
  \red{RISCRITTO E CORRETTO FINO A QUI}
\end{center}
\bigskip




\paragraph{It would be much better \dots } 
\cyan{QUI NON SONO SICURO SE \`E POSSIBILE SCEGLIERE IL CUBO DI INTEGRAZIONE IN
  MANIERA CORRETTA! QUELLO CHE VORREMMO }

If, finally, we COULD choose $U = A^{-1} \left( \{ x \in \R^g \, : \,
  |x|_\infty \leq N+\delta /2 \} \right)$ \cyan{(this is NOT a straight
  cube!)}, we would be able to refine \eqref{Birkhoff_sums_theta} as
\[
\lin \, _\alpha L ^U (m) , \Phi \rin = \frac{1}{|U|} \sum_{ n \in \Z^g \, , \,
  \, |n| \leq N} \varphi \left( e^{-\pi i X n\cdot n -2\pi i y \cdot n} \right)
\, .
\]

and therefore we would have proven the more elegant
  
\begin{conjecture}\label{theta_sums} For almost all $X \in \Sym_g(\R)$ and $p
  \in \R^g$, the Riemann-Siegel theta sums satisfy
  \[
  \sum _{n \in \Z^g \, , \, |n| \leq N} e^{\pi i Xn \cdot n + 2\pi i pn} =
  \mathcal O \left( N^{\frac{g}{2}-\varepsilon} \right) \] as $N \to \infty$,
  for any $\varepsilon >0$.
\end{conjecture}


\bigskip

\cyan{Qui si potrebbe aggiungere il risultato ``if $\GMod \alpha$ is of bounded
  type, then \dots ''}

